Randomized Revenue Monotone Mechanisms for Online Advertising

Online advertising is the main source of revenue for many Internet firms. A central component of online advertising is the underlying mechanism that selects and prices the winning ads for a given ad slot. In this paper we study designing a mechanism for the Combinatorial Auction with Identical Items (CAII) in which we are interested in selling $k$ identical items to a group of bidders each demanding a certain number of items between $1$ and $k$. CAII generalizes important online advertising scenarios such as image-text and video-pod auctions [GK14]. In image-text auction we want to fill an advertising slot on a publisher's web page with either $k$ text-ads or a single image-ad and in video-pod auction we want to fill an advertising break of $k$ seconds with video-ads of possibly different durations. Our goal is to design truthful mechanisms that satisfy Revenue Monotonicity (RM). RM is a natural constraint which states that the revenue of a mechanism should not decrease if the number of participants increases or if a participant increases her bid. [GK14] showed that no deterministic RM mechanism can attain PoRM of less than $\ln(k)$ for CAII, i.e., no deterministic mechanism can attain more than $\frac{1}{\ln(k)}$ fraction of the maximum social welfare. [GK14] also design a mechanism with PoRM of $O(\ln^2(k))$ for CAII. In this paper, we seek to overcome the impossibility result of [GK14] for deterministic mechanisms by using the power of randomization. We show that by using randomization, one can attain a constant PoRM. In particular, we design a randomized RM mechanism with PoRM of $3$ for CAII.

==> discussion.tex <==
\section{Discussion and Future Works}
Note that our mechanism satisfies the desired IC property and gets a good portion of the maximum social welfare. However, one may worry that by enforcing revenue monotonicity we may lose in total revenue since it is an additional constraint. To address this issue, firstly, we emphasize that lack of revenue-monotonicity can lead to loss of revenue and efficiency from second-order effects that could be much higher than leaving some revenue to attain this property. Most teams in a technology firm treat auction as a black box without knowledge of its internal procedures. For example, assume a team designs a new
innovative ad format that increases the click-through-rate of certain ads. Without revenue-monotonicity, such changes can actually lower the revenue. The problem now is that this can result in this innovative change not getting into production system as it might be seen as a {\em bad} change. This can be a real problem in practice, and as
auction designers, we need to address this problem. Secondly, our
ultimate goal is indeed to design auctions that satisfy good
properties in different dimensions including total revenue. However,
one must realize that almost nothing is known theoretically about this
important property of {\em revenue-monotonicity}. Therefore, to fully
understand it formally, in our model, we isolate and just focus on RM
property while maximizing social welfare. This work can be a starting point for the community to build
more results around RM property, and hopefully a general framework to
design RM mechanisms emerges.  Once we have the state of the art
understanding of RM, the next goal is to understand more objectives
simultaneously.
